Layout Decomposition for Quadruple Patterning Lithography and Beyond

For next-generation technology nodes, multiple patterning lithography (MPL) has emerged as a key solution, e.g., triple patterning lithography (TPL) for 14/11nm, and quadruple patterning lithography (QPL) for sub-10nm. In this paper, we propose a generic and robust layout decomposition framework for QPL, which can be further extended to handle any general K-patterning lithography (K$>$4). Our framework is based on the semidefinite programming (SDP) formulation with novel coloring encoding. Meanwhile, we propose fast yet effective coloring assignment and achieve significant speedup. To our best knowledge, this is the first work on the general multiple patterning lithography layout decomposition.

==> doc/app_graph.tex <==

\section{More on 3-Cut Removal}

In this section, we discuss more about the GH-tree based 3-cut removal.

\subsection{Additional Stitch Reduction}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.44\textwidth]{MPL_example2}
  \caption{Additional stitch in 3-cut removal.}
  %Example of additional stitch.~(a) Two stitch candidates (a,d) (b,e) in the 3-cut;
  %~(b) Color assignments on two components;
  %~(c) Rotate the colors and interconnect edges back, but one additional stitch is introduced.}
  %~(c) One additional stitch after color rotation.}
  \label{fig:example_2stitch_cut}
  \vspace{-.1in}
\end{figure}

Although 3-cut removal is safe without additional conflict, it might introduce additional stitches when there are more than one stitch candidates in the 3-cut.
%Kuang et al. \cite{TPL_DAC2013_Kuang} pointed out that
An example is illustrated in Fig. \ref{fig:example_2stitch_cut} (a), where two stitch candidates ($a-d, b-e$) are within a 3-cut.
After color assignment on the two components, vertices $a, b$ are assigned the same color, while colors of $d, e$ are different.
No matter how to rotate the colors, one additional stitch would be introduced (see Fig. \ref{fig:example_2stitch_cut} (c)). 
To restrict the stitch number of each 3-cut, we associate all stitch edges with higher weight ($1.4$).
After GH-tree construction, a weight refinement is proposed to round all edge weights to the first decimal for discrete values.
%to round all edge weights.
If there is only one stitch candidate, the weight of a 3-cut is $3.4$, which would be rounded down to $3$.
Otherwise, if there are two stitch candidates, the corresponding weight $3.8$ would be rounded up to $4$.
%By this way, if there are two stitch candidates in the 3-cut, we pay some penalty to its weight.
%Take the graph in Fig. \ref{fig:example_2stitch_cut} (a) as example, because of the two stitch edges, the weight of the three edges would be rounded up to $4$.
For instance in Fig. \ref{fig:example_2stitch_cut} (a), the weights of three edges are rounded up to $4$ as a result of two stitch edges.
Therefore, these three edges would not be removed as a 3-cut during graph division.

% ============ GH-Tree Experiment ==============
\subsection{Effectiveness of GH-Tree}

% table 2: effectiveness of GH-tree
\begin{table}[tb]
\centering
%\renewcommand{\arraystretch}{0.9}
\caption{Effectiveness of GH-tree for QPLD}
%{{{
  \label{tab:ghtree}
  \begin{tabular}{|c|ccc|ccc|}
    \hline \hline
    \multirow{2}{*}{Circuit}
    &\multicolumn{3}{c|}{SDP w/o. GH-tree }
    &\multicolumn{3}{c|} {SDP w. GH-tree}\\
    \cline{2-7}
    &cn\#  &st\#     &CPU(s)
    &cn\#  &st\#     &CPU(s) \\
    \hline                                                                                      
    C432         &2   &1       &0.2                            &2     &1       &0.1   \\
    C499         &1   &4       &0.3                            &1     &4       &0.2   \\
    C880         &1   &3       &0.2                            &1     &3       &0.1   \\
    C1355        &0   &4       &0.1                            &0     &4       &0.1   \\
    C1908        &2   &3       &0.4                            &2     &3       &0.3   \\
    C2670        &0   &7       &0.4                            &0     &8       &0.2   \\
    C3540        &1   &7       &0.4                            &1     &7       &0.3   \\
    C5315        &1   &18      &1.1                            &1     &20      &0.6   \\
    C6288        &21  &1       &1.5                            &21    &1       &1.2   \\
    C7552        &3   &15      &1.1                            &3     &15      &0.8   \\
    S1488        &0   &0.8     &0.6                            &0     &0.8     &0.4   \\
    S38417       &31  &553     &41.9                           &31    &557     &33.9  \\
    S35932       &105 &1764    &182.3                          &105   &1765    &141.8 \\
    S38584       &81  &1675    &167.7                          &81    &1679    &130.2 \\
    S15850       &78  &1472    &152.0                          &78    &1477    &110.7 \\
    \hline
    avg.         &21.8&369.0   &36.7                           &21.8  &370.1   &28.1  \\
    ratio        &\textbf{1.0}   &\textbf{1.0}      &\textbf{1.0}
                 &\textbf{1.0}   &\textbf{1.003}    &\textbf{0.77} \\
    \hline \hline
  \end{tabular}
%}}}
\end{table}

To demonstrate the effectiveness of the GH-tree based 3-cut removal, we compare two SDP based frameworks ``\textbf{SDP w. GH-tree}'' and ``\textbf{SDP w/o. GH-tree}'',
where ``SDP w. GH-tree'' integrates GH-tree based cut removal into the graph division stage, while ``SDP w/o. GH-tree'' does not apply GH-tree technique.
It shall be noted that all division techniques for double/triple patterning have been applied to both frameworks.
Here $min_s$ is set as 85nm.
As shown in Table \ref{tab:ghtree}, through applying GH-tree based graph division, our framework can reduce the runtime by 23\%.
The reason is that through 3-cut removal, each divided graph component tends to have smaller size, therefore have less runtime in corresponding color assignment.
In addition, ``SDP w. GH-tree'' can maintain the same conflict number, while the stitch number is very comparable (only 0.3\% of difference) with ``SDP w/o. GH-tree''.
%We conclude that by Table \ref{tab:ghtree} GH-tree based graph division is highly efficient and effective in terms of complexity reduction and solution quality.





==> doc/app_ilp.tex <==

\section{ILP based Color Assignment}
\label{sec:app_ilp}

In this section, we discuss how integer linear programming (ILP) can be applied to solve the color assignment in QPLD.
The general mathematical formulation is shown in (\ref{eq:math}).

\begin{align}
  \textrm{min}  	&     \ \ \ \  \sum_{e_{ij} \in CE} c_{ij} + \alpha \sum_{e_{ij} \in SE}s_{ij}&   \label{eq:math}\\
  \textrm{s.t}.\ \
  & c_{ij} \leftarrow ( x_i = x_j )		&\forall e_{ij} \in CE		\label{matha}\tag{\ref{eq:math}$a$}\\
  & s_{ij} \leftarrow x_i \oplus x_j	&\forall e_{ij} \in SE		\label{mathb}\tag{\ref{eq:math}$b$}\\
  & x_i \in \{0, 1, 2,3\}			    & \forall i \in V			\label{mathc}\tag{\ref{eq:math}$c$}
\end{align}
where $x_i$ is a variable for the three colors of rectangles $r_i$,
$c_{ij}$ is a binary variable for conflict edge $e_{ij} \in CE$ and $s_{ij}$ is a binary variable for stitch edge $e_{ij} \in SE$. 
Constraint (\ref{matha}) is used to evaluate the conflict number when touch vertices $r_i$ and $r_j$ are assigned different colors (masks).
Constraint (\ref{mathb}) is used to calculate the stitch number. If vertices $r_i$ and $r_j$ are assigned the same color (mask), stitch $s_{ij}$ is introduced.


Inspired by \cite{TPL_ICCAD2011_Yu}, the mathematical formulation in (\ref{eq:math}) can be solved through integer linear programming (ILP) as in (\ref{eq:ILP}).

\begin{figure}[h]
\vspace{-.1in}
\begin{align}
\textrm{min}  &  \sum_{e_{ij} \in CE} c_{ij} + \alpha \sum_{e_{ij} \in SE}s_{ij} 		\label{eq:ILP}\\
\textrm{s.t}.\ \
  &	x_{i1}+x_{j1}-c_{ij1} \le 1,     \ \  x_{i1}+x_{j1}+c_{ij1} \ge 1          \label{ILPa}\tag{\ref{eq:ILP}$a$}\\
  &	x_{i2}+x_{j2}-c_{ij2} \le 1,     \ \  x_{i2}+x_{j2}+c_{ij2} \ge 1          \label{ILPb}\tag{\ref{eq:ILP}$b$}\\
  &	c_{ij1} + c_{ij2} \le 1 + c_{ij} \ \  				                       \label{ILPc}\tag{\ref{eq:ILP}$c$}\\
  &	x_{i1}-x_{j1} \le s_{ij1},       \ \  x_{j1}-x_{i1} \le s_{ij1}            \label{ILPd}\tag{\ref{eq:ILP}$d$}\\
  &	x_{i2}-x_{j2} \le s_{ij2},       \ \  x_{j2}-x_{i2} \le s_{ij2}            \label{ILPe}\tag{\ref{eq:ILP}$e$}\\
  &	s_{ij} \ge s_{ij1},              \ \  s_{ij} \ge s_{ij2}			       \label{ILPf}\tag{\ref{eq:ILP}$f$}\\
  & x_{ij} \textrm{ is binary}       \ \                                       \label{ILPg}\tag{\ref{eq:ILP}$g$}
\end{align}
\vspace{-.3in}
\end{figure}


The objective function minimizes the weighted summation of the conflict number and the stitch number.
Constraints (\ref{ILPa}) -- (\ref{ILPc}) equal to constraint (\ref{matha}),
where 0-1 variable $c_{ij1}$ demonstrates whether $x_{i1}$ equals to $x_{j1}$, and $c_{ij2}$ demonstrates whether $x_{i2}$ equals to $x_{j2}$.
0-1 variable $c_{ij}$ is true only if two vertices connected by conflict edge $e_{ij}$ are in the same color, e.g. both $c_{ij1}$ and $c_{ij2}$ are true.
Constraints (\ref{ILPd}) -- (\ref{ILPf}) equal to constraint (\ref{mathb}),
where 0-1 variable $s_{ij1}$ demonstrates whether $x_{i1}$ is different from $x_{j1}$, and $s_{ij2}$ demonstrates whether $x_{i2}$ is different from $x_{j2}$.
Stitch $s_{ij}$ is true if either $s_{ij1}$ or $s_{ij2}$ is true.

To overcome the possible runtime overhead of ILP,
a popular speedup technique is to relax the ILP into linear programming (LP) by removing the constraint (\ref{ILPg}).
%Although ILP can search the optimal solution theoretically, for practical design it may suffer from long runtime penalty.
It is obvious that the LP solution provides a lower bound to the ILP formulation.
However, we observe that the LP solution would be like this: each $x_{ij}$ is assigned to $0.5$.
By this way all the constraints are satisfied, and the objective function is minimized.
However, all these $0.5$ values provide no useful information to guide the color assignment,
since we prefer each $x_{ij}$ is closes to either $0$ or $1$.






==> doc/app_linear.tex <==

\section{More on Linear Color Assignment}
\label{sec:app_linear}

In this section, we discuss more about the linear color assignment.
As mentioned in Section \ref{sec:linear}, three different vertex orders are applied simultaneously in \textit{peer selection}.
We now introduce and compare the three orders.
\begin{enumerate}
  \item \textbf{SEQUENCE-COLORING}: Vertices are assigned colors based on the initial order.
  \item \textbf{DEGREE-COLORING}: Vertices are assigned colors based on a nearly conflict degree descending order.
  \item \textbf{3ROUND-COLORING}: Vertices are solved through conflict degree descending order.
        In addition, the vertex with only one legal possible color would be assigned first.
\end{enumerate}

Vector $vec$ is constructed to provide the vertices with conflict degree descending order.
Instead of completely sorting all vertices which needs $O(nlogn)$, vector $vec$ contains $vec$[1], $vec$[2], and $vec$[3], successively.
The vector $vec$[i], $1 \le i \le 3$, contains vertices with special conflict degree, defined as follows:
\begin{align}
  vec[1] = & \{v_i | \forall v_i \in V, d_{conf}(v_i) > 6\}        \notag\\
  vec[2] = & \{v_i | \forall v_i \in V, 4 < d_{conf}(v_i) <= 6\}   \notag\\
  vec[3] = & \{v_i | \forall v_i \in V, d_{conf}(v_i) <= 4\}       \notag
\end{align}
%That is, $vec$[1] is the set of vertices with conflict degree larger than 6, $vec$[3] is the set of vertices with conflict degree 4 or less,
%and $vec$[2] contains all other vertices.
The main idea is that the vertices in $vec$ are nearly conflict degree descending order, but the construction is in linear time.


\begin{algorithm}[htb]
\caption{3ROUND-COLORING($vec$)}
\label{alg:3round}
%{{{
\begin{algorithmic}[1]
  \Require Vector $vec$ containing all vertices;
  \State Label each $v_i \in vec$ as UNSOLVED;
  \ForAll {vertex $v_i \in vec$}               \Comment{1st round}
    \State $c(v_i) \leftarrow$ a minimum cost color;
    \State Label $v_i$ as SOLVED;
    \If{All four colors have been applied at least once}
      \State Break;                            \Comment{End 1st round}
    \EndIf
  \EndFor
  \ForAll {UNSOLVED vertex $v_i \in vec$}      \Comment{2nd round}
    \If{$v_i$ has only one legal color c}
      \State $c(v_i) \leftarrow$ c;
      \State Label $v_i$ as SOLVED;
    \EndIf
  \EndFor
  \ForAll {UNSOLVED vertex $v_i \in vec$}      \Comment{3rd round}
    \State $c(v_i) \leftarrow$ a minimum cost color;
      \State Label $v_i$ as SOLVED;
  \EndFor
  \State \Return {$c(v_i), \forall v_i \in vec$;}
\end{algorithmic}
%}}}
\end{algorithm}


The details of the method \textit{3ROUND-COLORING} are shown in Algorithm \ref{alg:3round},
where the vertex with less coloring choices tends to be resolved first.
In other words, we prefer to assign color to a vertex with ``less flexibility''.
At the beginning, all vertices are labeled as UNSOLVED (line 1), then the vector $vec$ is scanned thrice.
In the first round scanning, for each vertex $v_i \in vec$, a greedy color with minimum cost would be assigned (lines 2-4).
When all four colors have been applied at least once, the first round is stopped.
In the second round scanning, only those vertex with only one legal color would be assigned color.
By this way, we prefer to assign colors to those vertices with ``less flexibility''.
When a vertex is assigned one color, it is labeled as SOLVED.
In the third scanning, we greedily assign colors to those UNSOLVED vertices.

\iffalse
\begin{algorithm}[h]
\label{alg:sequence}
%{{{
\begin{algorithmic}[1]
  \Require Queue $Q$ containing all vertices;
  \For{aa}
    \State haha
  \EndFor
\end{algorithmic}
%}}}
\end{algorithm}
\fi

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.44\textwidth]{MPL_cnf_compare}
  \caption{Comparison on conflict number.}
  \label{fig:cnf_compare}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.44\textwidth]{MPL_stt_compare}
  \caption{Comparison on stitch number.}
  \label{fig:stt_compare}
\end{figure}

Fig. \ref{fig:cnf_compare} and Fig. \ref{fig:stt_compare} compare the performance of different vertex orders,
in terms of the conflict number and the stitch number.
Here \textit{SEQUENCE-COLORING}, \textit{DEGREE-COLORING}, and \textit{3ROUND-COLORING} denote the coloring through three different orders, respectively.
\textit{Peer-Selection} is the method proposed in our linear color assignment. 
From Fig. \ref{fig:cnf_compare} we can clearly see that peer selection can achieve less conflict number than any single vertex order.
The reason is that, for each test case, the whole decomposition graph would be divided into several components.
For each component one specific order may be dominant, then this order would be adopted by peer selection scheme.
Therefore, for the whole layout, peer selection would be better than any single vertex ordering rule.




==> doc/app_proof.tex <==

\section{Proof of Lemmas}
\label{sec:app_proof}

\noindent
\underline{PROOF OF LEMMA \ref{lem:3cut}}
\begin{proof}
We denote the three edges in a 3-cut as ($a_1-b_1, a_2-b_2, a_3-b_3$).
Without loss of generality, we rotate the colors of ${b_1, b_2, b_3}$ to remove any conflict derived on the edges.
%c($b_1$), c($b_2$), and c($b_3$) are denoted the assigned colors of $b_1$, $b_2$ and $b_3$, respectively.
%Here c($b_1$), c($b_2$), c($b_3$) $\in \{0, 1, 2, 3\}$.
Since all vertices should be rotated by the same value, there are four rotation options for the whole component.
%Since there are four possible color choices, during color rotation, every vertex has four rotation options.
For one edge $\{a_1-b_1\}$, one option is infeasible that would causes one conflict.
At most three options are infeasible on the 3-cut.
Therefore, at least one option left is feasible without any conflict introduced on the 3-cut.
%Therefore, at least one option left is okay that no conflict is introduced on the 3-cut.
\end{proof}


%\noindent
%\underline{PROOF OF THEOREM \ref{thm:ksdp}}
%\begin{proof}
%TO BE CONTINUED ...
%\end{proof}




==> doc/bak/app_fm.tex <==
\section{FM Partition Color Assignment}

ILP suffers from serious runtime overhead, while corresponding LP relaxation may be not good in terms of performance.
Therefore, we propose an FM partition heuristic to provide faster color assignment solution.
In decomposition graph (DG), if each edge in $CE$ is associated with weight $1$, while each edge in $SE$ is associated with weight $-\alpha$,
then the QPLD problem is a four-way maximum cost partition on the DG.
Since maximum cost partition is NP-hard, we propose a fast heuristic method,
which is extended from FM partition \cite{PAR_DAC82_FM}.
Note that FM partition has been applied in double/triple patterning problems \cite{DPL_ASPDAC2010_Yang,TPL_ISQED2013_Chen}.


\begin{algorithm}[tb]
\caption{FM Partition Color Assignment}
\label{alg:fm}
\begin{algorithmic}[1]
  \State Randomly generate initial color assignment;
  \State Compute gains of all nodes;
  \While {$Improve = TRUE$}
    \While {exist unlock nodes}
      \State Select node $n_i$ with maximum gain $g_i$;
      \State Assign one color to $n_i$ and lock $n_i$;
      \State Update gains of all unlock nodes;
    \EndWhile
    \State Select best sequence of color assignments, $s.t., G = \sum g_i$ is maximum;
    \State Assign color to the sequence;
    \If {$G \le 0$}
      \State $Improve \leftarrow FALSE$;
    \Else
      \State $Improve \leftarrow TRUE$;
    \EndIf
    \State Free all nodes;
  \EndWhile
\end{algorithmic}
\end{algorithm}

The details of our FM partition is shown in Algorithm \ref{alg:fm}.
Our algorithm performs passes wherein each model moves exactly once,
returns the best solution observed during a pass, and terminates when a pass fails to improve the cost function.
Time complexity of our heuristic is linear.
In practice only a very small number of passes are required.



==> doc/bak/overview.tex <==

\section{Overview of Layout Decomposition Flow}
\label{sec:overview}

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.48\textwidth]{overview}
  \caption{~Proposed layout decomposition flow.}
  \label{fig:overview}
\end{figure}


The overall flow of our layout decomposition is highlighted in Fig. \ref{fig:overview}.
Given input layout and minimum coloring distance $min_s$,
we first construct decomposition graph (DG) to transform the original geometric problem into a graph problem.
By this way, the QPLD problem can be modeled as 4 color assignment on the DG.
To reduce the problem size, graph division techniques (see Section \ref{sec:graph}) are applied to partition the DG into a set of components.
Then the color assignment problem can be solved independently for each component.
In order to assign color, in Section \ref{sec:algo} we propose a set of algorithms, i.e., integer linear programming (ILP) formulation,
FM partition, and semidefinite programming (SDP) based algorithm.




==> doc/bak/problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

%In this section we introduce the problem formulation.
%Given input layout which is specified by features in polygonal shapes, a \textit{layout graphs} (LG) is constructed.
Given a layout featured in polygon shapes, a \textit{layout graph} (LG) is constructed by Definition \ref{def:lg}.

\begin{mydefinition}[Layout Graph]
\label{def:lg}
% === defined by Tsung-Wei
A layout graph (LG) is an undirected graph in which vertex set represents the polygonal shapes and edge set represents the connection if and only if the two corresponding polygonal shapes are within minimum coloring distance $min_s$.
%The layout graph (LG) is an undirected graph whose vertices are the given layout's polygonal shapes and where an edge exists if and only if the two polygonal shapes are within minimum coloring distance $min_s$ of each other.
\end{mydefinition}

We use Fig. \ref{fig:LG2DG} for illustration.
An input layout example is shown in Fig. \ref{fig:LG2DG} (a) and its corresponding LG is constructed as in Fig. \ref{fig:LG2DG} (b).
Based on the LG, vertex projection is performed to search all stitch candidates.
Then the LG will be transferred into a \textit{decomposition graph} (DG) to store all the LG information and the stitch candidates.
%Note that different from the decomposition graph in \cite{TPL_ICCAD2011_Yu} where only double patterning stitch candidates are selected,
Note that in vertex projection we choose all the possible stitch candidates as described in \cite{TPL_DAC2013_Kuang}.

\begin{mydefinition}[Decomposition Graph]
A decomposition \\ graph (DG) is an undirected graph $\{V, CE, SE\}$ with a single set of vertices $V$,
and two edge sets $CE$ and $SE$ containing the \textit{conflict edges} (CE) and \textit{stitch edges} (SE), respectively.
Each vertex  $v \in V$ represents a polygonal shape, an edge $e \in CE$ exists iff the two polygonal shapes are within minimum coloring distance $min_s$,
and an edge $e \in SE$ iff there is a stitch candidate between the two vertices which are associated with the same polygonal shape.
\end{mydefinition}

% LG / DG Figure
\begin{figure}[tb]
  \centering
  \subfigure[] {\includegraphics[width=0.14\textwidth]{LG2DG1}}
  \subfigure[] {\includegraphics[width=0.15\textwidth]{LG2DG2}}
  \subfigure[] {\includegraphics[width=0.17\textwidth]{LG2DG3}}
  \caption{~(a) Input layout;~(b) Layout graph (LG);~(c) Decomposition graph (DG).}
  \label{fig:LG2DG}
\end{figure}

With two stitch candidates, the LG in Fig. \ref{fig:LG2DG}(b) will be transferred into a DG (see Fig. \ref{fig:LG2DG}(c)).
Please refer to \cite{DPL_ISPD2010_Xu,TPL_ICCAD2011_Yu} for more details regarding the decomposition graph (DG).
Based on DG, we carry out color assignment to assign all the vertices into four masks (colors).
%The layout decomposition is called quadruple patterning layout decomposition.

We define the quadruple patterning layout decomposition (QPLD) problem as follows:

\begin{myproblem}[QPLD]
Given an input layout which is specified by features in polygonal shapes and minimum coloring distance $min_s$,
the decomposition graph (DG) is constructed.
Quadruple patterning layout decomposition (QPLD) assigns all the vertices in DG into one of four colors (masks) to minimize conflict number and stitch number.
\end{myproblem}

The QPLD problem can be extended to general K-patterning layout decomposition problem as follows.

\begin{myproblem}[K-Patterning Layout Decomposition]\ \\
Given an input layout, the decomposition graph (DG) is constructed.
Each vertex in DG would be assigned into one of K colors (masks) to minimize conflict number and stitch number.
\end{myproblem}

% =================================================================
%                         NP-hardness
% =================================================================
\iffalse
At the first glance, QPLD problem can be solved through \textit{four color map theorem}\cite{1977Appel} that every planar graph is 4-colorable.
However, we observe that in emerging technology node, the designs are so complex that for most cases the layout graphs are not planar.
In addition, we have the following lemma that inserting stitch cannot planarize the graph.

\begin{mylemma}
\label{lem:planar}
If a layout graph (LG) is not planar, after stitch candidate insertion, the corresponding decomposition graph (DG) is still not planar.
\end{mylemma}

The proof can be based on \textit{Kuratowski's theorem} \cite{1930Kuratowski} that
a finite graph is planar iff it does not contain a subgraph that is a subdivision of $K_5$ or of $K_{3,3}$.
Here $K_5$ is the complete graph on five vertices, while $K_{3,3}$ is the complete bipartite graph on six vertices (three on each side).
Due to space limit, the detailed proof is omitted.

It has been shown that triple patterning layout decomposition, which is a $3$ patterning problem, is NP-hard \cite{TPL_ICCAD2011_Yu}.
Besides, since triple patterning layout decomposition can be polynomial-time reducible to QPLD,
QPLD problem is NP-hard as well.
In addition, we can get the conclusion that general K-patterning layout decomposition problem, with $K \ge 3$, is NP-hard.
\fi


